Data Level Lottery Ticket Hypothesis for Vision Transformers

The conventional lottery ticket hypothesis (LTH) claims that there exists a sparse subnetwork within a dense neural network and a proper random initialization method called the winning ticket, such that it can be trained from scratch to almost as good as the dense counterpart. Meanwhile, the research of LTH in vision transformers (ViTs) is scarcely evaluated. In this paper, we first show that the conventional winning ticket is hard to find at the weight level of ViTs by existing methods. Then, we generalize the LTH for ViTs to input data consisting of image patches inspired by the input dependence of ViTs. That is, there exists a subset of input image patches such that a ViT can be trained from scratch by using only this subset of patches and achieve similar accuracy to the ViTs trained by using all image patches. We call this subset of input patches the em winning tickets, which represent a significant amount of information in the input data. We use a ticket selector to generate the winning tickets based on the informativeness of patches for various types of ViT, including DeiT, LV-ViT, and Swin Transformers. The experiments show that there is a clear difference between the performance of models trained with winning tickets and randomly selected subsets, which verifies our proposed theory. We elaborate on the analogical similarity between our proposed Data-LTH-ViTs and the conventional LTH to further verify the integrity of our theory. The Source codes are available at https://github.com/shawnricecake/vit-lottery-ticket-input.

==> sections/7_resubmission.tex <==



\section{Reviewer's Comments}

\subsection{Reviewer 1}


\noindent\textbf{Q1:} Effectively, a winning set of tokens implies that the attention is always sparse in the vision transformer. While this is generally true, how does it hold in case the attention is not sparse?

\noindent\textbf{R1:} The patches included in the winning set can also contribute to the attention, but the contribution is not as large as the winning patches because the accuracy can be optimized when we increase the number of patches left in the winning set. Therefore, the vision transformer can receive additional information from the attention when we increase the number of patches, which means that the attention mechanism is the same whenever it is sparse or dense.


\noindent\textbf{Q2:} The authors have compared Deit-small on Imagenet (Table-1) vs. Resnet-20 on CIFAR-10 (Table-2). It would be nice to keep the dataset the same and vary the model for a fair and convincing comparison.

\noindent\textbf{R2:} We follow the traditional lottery ticket hypothesis to build our experiments of ResNet-20 on CIFAR-10, which is mainly used to show the LTH on CNNs and the influence of the rewinding technique.
Actually, some works[sanity check of LTH] indicate that the weight level winning ticket is hard to find with CNNs on the ImageNet dataset, even with the rewinding technique. Therefore, we did not show the weight level LTH results on ImageNet.
On the other hand, the resolution has a notable effect on the training of ViTs, and we need to rescale the input resolution from 32 to 224 if we need to do the experiments on the CIFAR-10 dataset, which is unfair to compare with the CNNs. Besides, if we keep the input resolution at 32, we need to use transfer learning, preventing us from training the model from scratch.


\noindent\textbf{Q3:} Is there any particular reason why the rewinding results have not been reported for 53\% sparsity in Table 1?

\noindent\textbf{R3:} As the rewinding experiments need much time, we use 3 different sparsity ratios, and the weight sparsities are 26\%, 44\%, and 71\%. The experimental results at 26\% weight sparsity are the following:
LTH Acc.: 78.58\%,
RR Acc.: 78.76\%,
Acc. Diff.: -0.18,


\noindent\textbf{Q4:} The authors mentioned, 'Transformer is first introduced to the computer vision research area by (Dosovitskiy et al. 2021).' Factually this is incorrect. The first impactful application in vision was made by Carion et al. [1].


\noindent\textbf{R4:} Thanks for pointing that out. We will correct this in the revision.





\subsection{Reviewer 2}

\noindent\textbf{Q1:} First, I do not think LTH is related to the topic of the proposed method. I think the proposed “Patch LTH” is similar to data value [1]/data efficient [2,3] in the CNNs. I think a more suitable topic is “patch-efficient ViTs”. Furthermore, different from conventional LTH that suggests winning tickets found in CNN have connections with the initial weights that can make the training particularly effective, the so-called patch LTH is not the only one. Adopting Random Choice to part of the training data may have the similar performance to Winning Lottery ticket. In summary, I do not think the topic of this paper is LTH.


\noindent\textbf{R1:} We do not claim any efficiency of our method in the paper. What we propose is that the vision transformers have a connection with the winning patches that can make the training particularly effective, which is the main reason that we define the topic of our paper as a new kind of LTH. Our results in Figure 3 have clearly shown superior accuracy when using winning patches over the Random Choice in model training.


\noindent\textbf{Q2:} My main concern is the contribution of the proposed patch LTH of ViTs. The motivation of this paper is efficient training and test (inference) of ViT models. However, the ticket selector in this paper is not an efficient processing, which needs a pretrained ViT. Furthermore, as shown in Table 4, the acquired winning tickets seem to have Limited generalization to different ViTs. Therefore, I don't think it's efficient if I need a full pre-training before I can train a model efficiently.

\noindent\textbf{R2:} Our motivation is not efficient training and testing of ViT models. We claim the effectiveness of patch sparsity, which follows both the motivation and process of conventional LTH (using a pretrained model to find a kind of sparse pattern for effective training), except that our LTH is applied to patch instead of weight, which has never been explored before. As for the generalization to Swin Transformer in Table 4, we have explained that the inattentive patches are occluded with all-zero value (black color) instead of removing them, which is caused by the input restriction (input image must be the square size) of the Swin Transformer. Therefore, the training or test input for the Swin Transformer is still sparse because of the black occlusion.




